Supernova remnants in the very-high-energy gamma-ray domain: the role of the Cherenkov telescope array

Supernova remnants are often presented as the most probable sources of Galactic cosmic rays. This idea is supported by the accumulation of evidence that particle acceleration is happening at supernova remnant shocks. Observations in the TeV range have especially contributed to increase the understanding of the mechanisms, but many aspects of the particle acceleration at supernova remnant shocks are still debated. The Cherenkov telescope array is expected to lead to the detection of many new supernova remnants in the TeV and multi-TeV range. In addition to the individual study of each, the study of these objects as a population can help constrain the parameters describing the acceleration of particles and increase our understanding of the mechanisms involved.

==> 00README.XXX.tex <==
nohypertex
